The Majority Can Help The Minority: Context-rich Minority Oversampling for Long-tailed Classification

The problem of class imbalanced data is that the generalization performance of the classifier deteriorates due to the lack of data from minority classes. In this paper, we propose a novel minority over-sampling method to augment diversified minority samples by leveraging the rich context of the majority classes as background images. To diversify the minority samples, our key idea is to paste an image from a minority class onto rich-context images from a majority class, using them as background images. Our method is simple and can be easily combined with the existing long-tailed recognition methods. We empirically prove the effectiveness of the proposed oversampling method through extensive experiments and ablation studies. Without any architectural changes or complex algorithms, our method achieves state-of-the-art performance on various long-tailed classification benchmarks. Our code is made available at https://github.com/naver-ai/cmo.

==> 2-Introduction-WIP.tex <==
\section{Introduction}
\label{sec:intro}
%1문단. Target task: Long-tailed classification (imbalanced data) 의 어려움과 문제점

\begin{figure}[t]
\centering{%
\includegraphics[width=1\columnwidth]{latex/figures/images/concept_summary.pdf}}
\caption{\textbf{Concept of proposed minority oversampling}.
In the real-world long-tailed dataset iNaturalist 2018~\cite{ref:data_iNat}, the number of samples from head class and tail class is extremely different.
Naive random oversampling method repeatedly produces similar images from minority classes.
We propose a novel oversampling for generating diversified minority images by using various contexts from majority samples.}
\label{fig:concept}
\end{figure}

Solving data imbalance problem is important since real-world data are likely to be inherently imbalanced~\cite{ref:data_celeba, ref:data_coco, ref:data_uci, ref:data_iNat}.
Models trained on such imbalanced dataset are inevitably biased to majority classes than the minority classes, which leads to overfitting problem. 
% Besides, high-capacity deep neural networks (DNNs) can memorize samples from minority classes~\cite{ref:arpit_memoriz_icml2017} before learning generalized representations, which leads to the overfitting problem with high generalization error.


A simple and straightforward method to overcome the data imbalance is to repeatedly over-sample the minority classes~\cite{ref:resample_chawla_smote02,ref:resample_hulse_icml07}. However, those naive oversampling may rather intensify the overfitting problem since the repeatedly selected samples have less diversity with almost similar image contexts. For example, consider a minority class of ducks where the ducks always stand upon grasses in the training images. (See Figure 1?) 


% 2-3문단 suggestion (지금 버전도 좋은데 조금 related work 으로 넘기고 간결하게 가는것도 좋아보입니다)
% - the most simple and straightforward method to overcome imbalanced dataset problem = minority class oversampling (\cite{ref:resample_chawla_smote02}, \cite{ref:resample_hulse_icml07})
% (GAN-based, meta-learning-based 방법과 비교는 related work 으로 이동)
% - their problem: cannot ensure diversity of the samples from minority classes since they repeatedly select samples
% - repetitive samples (lack of diversity) can rather intensify over-fitting of a model. 
% - we propose a simple oversampling method thatcan generate diverse minority samples.
% - our method directly balances the training data distributions -> so our method can be easily combined with class re-weighting methods. 
% (class re-weighting 문헌들도 related work 으로 이동)


% 2문단. Previous Literature
% 크게 2가지 re-weighting, re-sampling. 
% Re-weighting: Assign different weights to each sample according to its importance.
% Re-sampling: Directly balance the training data distributions by re-sampling.
% re-sampling 방식이 직접적으로 데이터 불균형을 해결하는 방법이며, 데이터 불균형이 해결되면 꼭 re-weighting 방법을 안쓰고도 다른 일반적인 다양한 vision 문제 해결 method와 결합할 수 있기 때문에 이쪽을 해결하겠음. %Others: 최근 방식으로, meta-learning, two-stage,  ensemble 등 다양한 아키텍쳐와 트레이닝 테크닉 사용함-> related work에서 이야기.
% For decades, there have been various studies to handle the class imbalance problem~\cite{ref:anand_ranka_1993, ref:li_kdd_1998, ref:japkowicz_stehphen_2002, ref:He_Garcia_2009, ref:huang_tang_cvpr16, ref:cui_belongie_cvpr19, ref:zhou_chen_bbn_cvpr2020, ref:lade_cvpr2021, ref:ibloss_iccv2021}. 
% Methods for handling class imbalance are commonly divided into two major groups: class re-weighting and re-sampling.
% Class re-weighting approach re-weights samples according to their importance~\cite{ref:lin_focal_loss_iccv17, ref:cao_ldam_neurips2019, ref:cui_belongie_cvpr19} while re-sampling methods aim to directly balance the training distribution~\cite{ref:resample_hulse_icml07, ref:sankha_gamo_iccv2019}.
% In this work, we focus on the re-sampling method which solves the fundamental problem of the lack of minority classes.
% This is because when the imbalance of training data is resolved, it can be easily combined with various methods in computer vision tasks.  



% % 3문단. 기존의 Re-sampling approaches 문제점
% % ""심플하게 resampling vs. ours 로 놓고 label distribution 이 uniform 한 것은 동일하지만 image pixel level 로 갖는 context info 가 차이가 난다"" 요 흐름.
% % 강조하고 싶은 것: (1) 어느 task에 쉽게 결합할 수 있는 쉬운 minority over sampling 방법
% % (2) 기존 방법들처럼 minority 내에서 interpolate 하는 것이 아닌, majority class의 rich information 이용해서 다양한 sample 만든다.
% Despite the importance, the re-sampling approach has not received much attention compared to the other approaches in the community.
% It is because recent minor-oversampling methods are computationally expensive and difficult to be incorporated into deep learning algorithms for various computer vision tasks.
% For example, to generate new samples from minority classes, Generative Adversarial Networks (GAN) based methods~\cite{ref:sankha_gamo_iccv2019, ref:ewgan_aaai2019} require training generators, while meta-learning based methods~\cite{ref:metasaug_cvpr2021} demand additional balanced samples with hundreds and thousands of training iterations.
% Due to such practical challenges, classical methods such as SMOTE~\cite{ref:resample_chawla_smote02} which produces synthetic minority samples by interpolating between nearest images, or simple random oversampling (ROS)~\cite{ref:resample_hulse_icml07} are often used in practice.
% However, these methods cannot ensure diversity of newly created samples from minority classes since they repeatedly select samples with similar context at the pixel-level (See Figure \ref{fig:concept} (a)).
% It is known that repetitive samples can rather intensify overfitting of a model~\cite{ref:sarafianos_eccv2018}. 
% To  address  the  aforementioned  problem, in this work, we propose a simple oversampling method that can generate diverse minority samples. 

% 4문단. Proposed Method: minority oversampling 방법 제안
% 바람직한 minority oversampling/augmentation은 같은 것이 반복되는 것이 아닌, 다양한 샘플을 생성하는 것임.
% 예를 들어 다양하다는 것은 내 관심있는 대상이 다양한 배경에서 다양한 크기로 나타나는 것. occlusion이 있기도 하고. 
% 이러한 샘플을 만들기 위해 우리는 long-tail distribution이 갖는 특성에 주목했음: 곧, majority class sample은 데이터가 풍부하고 다양한 정보를 가지고 있음.
% 따라서 minority sample에 대해 majority sample을 배경으로 활용하여 augmented sample을 만듬.
% Figure1은 우리가 제안하는 방법을 보여준다. 
A desirable minority oversampling is to generate a variety of samples that can induce a robust decision boundary.
To be diverse, the subject of our interest should appear in different sizes in various contexts. 
To make these samples, we pay attention to the characteristics of long-tailed distributions; that is, majority class samples are data-rich and information-rich.
Unlike the existing re-sampling methods that ignore (undersample) majority samples, we use the affluent information of the majority samples to generate new minority samples.
Specifically, our idea is to leverage the rich major-class images as the background for the newly created minor-class images.
Figure \ref{fig:concept} (b) illustrates the concept of our proposed oversampling strategy.
Given an original image from a minority class, the object is cropped in various sizes and pasted to the various images from majority classes. 
Then, we can create images with more diverse contexts than the existing oversampling methods that create synthetic images by interpolating within the minority classes.
Since this is an interpolation of the majority class and minority class samples, it generates diversified data around the decision boundary, and as a result, it helps to train a robust classifier.
To this end, we utilize Cutmix~\cite{ref:cutmix_iccv2019} which was proposed as a regularization strategy for training robust classifier.
However, naive use of CutMix may exacerbate the problem of long-tail distribution by generating more majority samples since majority samples are more likely to be selected.
We solve this problem by sampling the background images and the foreground patches from different distributions to achieve the desired minority oversampling.

%Inspired from recent success of CutMix~\cite{ref:cutmix_iccv2019} as an effective data augmentation strategy in various computer vision tasks, we utilize Cutmix which cut and paste patches among training images.
% 5문단. Contribution.
% 결과, Simple 해서 쉽게 사용하기 좋음. training cost 거의 안든다.
% CE에만 붙여도 많은 향상을 보였으며, LDAM 등 다른 loss와 결합했을 때 성능 향상 더 컸음. 

Our key contributions can be summarized as follows:
(1) We propose a novel \MakeLowercase{\ourfull} that generates various samples by leveraging the rich context of the majority classes as background images.
(2) Our method requires little additional training cost and can be easily integrated into various end-to-end deep learning algorithms for long-tailed recognition.
(3) We show that significant performance improvements can be achieved by adding the proposed oversampling to existing commonly used loss functions including cross-entropy loss and LDAM loss~\cite{ref:cao_ldam_neurips2019}. 
By adding only oversampling to the loss functions without any architectural changes or complex algorithms, it shows performance comparable to or surpassing recent state-of-the-art methods on various benchmark datasets.
(4) We empirically prove the effectiveness of the proposed oversampling method through extensive experiments and ablation studies.
We believe that our study can be a useful and universal minority oversampling method in long-tailed classification research.






% minority class 를 oversampling 하거나 artificial minority sample을 만들려는 방법들.
% random oversampling 등 training cost가 들지 않는 simple한 방법은 잘 동작 X, repetitive sample로 오히려 minority class overfitting 시킴.
% 아니면 생성은 효과적이어도 딥러닝 트레이닝에 결합하기 어려움.
% SMOTE, GAMO 등. 최근에 metasaug도 41
% “A number of informed oversampling techniques have also been developed to strengthen class boundaries, reduce over-ftting, and improve discrimination.” 
% <SMOTE: Synthetic Minority oversampling Technique> produces artifcial minority samples by interpolating between existing minority samples and their nearest minority neighbors.
% SMOTE는 아주 유명하고 classical machine learning 에서 많이 사용되는 방법. 이를 개선하기 위한 다양한 variant methods 도 나옴. 그러나 deep learning 에서 
% 한정적인 개수의 (몇 개 밖에 안되는 ) minority class 내에서 interpolation함 -> diverse 확보 어려움.
% GAN도 많은 발전이 있긴하지만, 트레이닝 어려우며, 다양하지 않고 특정 샘플을 생성하게 되는 mode collapse 문제는 잘 알려져있음.
% 이런 문제를 해결하기 위해 우리는 simple하면서 다양한 샘플을 생성할 수 있는 방법을 제안한다.

==> tables/old-cifar100-imb100.tex <==
% To-do: 다 업데이트 되고 나면 제일 좋은 값에 bold + Reference 달기. 
% 2021년 논문들이랑 비교를 하면 좀 더 확실하게 좋을 것 같음..

\begin{table}[]
\caption{
Classification accuracy (\%) of ResNet-32 on imbalanced CIFAR-100 with imbalance ratio of 100.
``$\dagger$" indicates that the results are copied from the original paper, 
and ``$\ddagger$" means that the results are from the experiments in RIDE~\cite{ref:ride_iclr2021}.
The best results are marked in bold.
}
\vspace{0cm}
\label{table:cifar100_imb100}
\centering
% \small
{
\begin{tabular}{lcccc}
\toprule
Methods                   & All  & Many & Med   & Few  \\ \midrule
Cross Entropy (CE)        & 38.6 & 65.3 & 37.5  & 8.7  \\
CE + Oversampling         & 32.3 & 55.3 & 30.9  & 7.0  \\
CE + Remix                & 40.0 & 71.7 & 38.5  & 4.9  \\
\rowcolor{lightcolor}
CE + Ours                 & 43.9 & 70.4 & 42.49 & 14.4 \\ \hline
BBN                       & -    & -    & -     & -    \\
Mixup (results from BBN)  & -    & -    & -     & -    \\
$\tau$-norm                 & 43.2 & 65.7 & 43.6  & 17.3 \\
cRT                       & 43.3 & 64.0 & 44.8  & 18.1 \\
RIDE (2 experts)          & 47.0 & 67.9 & 48.4  & 21.8 \\
2021 papers               & -    & -    & -     & -    \\ \hline
LDAM                      & 41.6 & 61.4 & 42.2  & 18.0 \\
LDAM + Oversampling       & 32.6 & 48.3 & 36.7  & 9.6  \\
LDAM + Remix              & 45.3 & 65.5 & 48.0  & 18.5 \\
\rowcolor{lightcolor}
LDAM + Ours               & 47.2 & 61.5 & 48.6  & 28.8 \\ \bottomrule
\end{tabular}
}
\end{table}

==> tables/old-cifar100.tex <==
\begin{table}[]
\caption{
Classification accuracy (\%) of ResNet-32 on imbalanced CIFAR-100-LT with different imbalance ratios.
``$\ast$" indicates that the results are copied from the original paper.
``$\dagger$ and $\ddagger$" means that the results are from ~\cite{ref:causalnorm_neurips2020} and \cite{ref:lade_cvpr2021}, respectively.
The best results are marked in bold.
}
\vspace{0cm}
\label{table:cifar100}
\centering
% \small
{
\begin{tabular}{lccc}
\toprule
Imbalance ratio         & 100  & 50   & 10   \\ \midrule
Cross Entropy (CE)        & 38.6 & 44.0 & 56.4 \\
CE + ROS~\cite{ref:resample_hulse_icml07}         & 32.3 & 39.7 & 55.6 \\
CE + Remix~\cite{ref:remix_eccv2020}                 & 40.0 & 45.0 & 58.7 \\
\rowcolor{lightcolor}
CE + Ours                 & 43.9 & 48.3 & 59.5 \\ 
CE-DRW        & 41.1 & 45.6 & 57.9  \\
CE-DRW + Remix~\cite{ref:remix_eccv2020}                & 45.8  & 49.5  & \textbf{61.7}  \\
\rowcolor{lightcolor}
CE-DRW + Ours                 & 47.0 & 50.9  & 59.2  \\ \hline
BBN~\cite{ref:zhou_chen_bbn_cvpr2020}$\dagger$                    & 42.6 & 47.1 & 59.2 \\
Causal Norm~\cite{ref:causalnorm_neurips2020}$\dagger$            & 44.1 & 50.3 & 59.6 \\
IB Loss~\cite{ref:ibloss_iccv2021}$^\ast$      & 45.0 & 48.9 & 58.0 \\
Balanced Softmax~\cite{ref:ren_bms_neurips2020}$\ddagger$ & 45.1 & 49.9 &61.6 \\
LADE~\cite{ref:lade_cvpr2021}$^\ast$      & 45.4 & 50.5 & \textbf{61.7} \\\hline
%MiSLAS~\cite{ref:mislas_cvpr2021}$\dagger$     & 47.0 & 52.3 & \textbf{63.2} \\ \hline
LDAM-DRW~\cite{ref:cao_ldam_neurips2019} & 41.7 & 47.9 & 57.3 \\
LDAM-DRW + ROS~\cite{ref:resample_hulse_icml07}   & 32.6 & 38.3 & 53.9 \\
LDAM-DRW + Remix~\cite{ref:remix_eccv2020}           & 45.3 & 48.8 & 55.9 \\
\rowcolor{lightcolor}
LDAM-DRW + Ours           & 47.2 & 51.7 & 58.4 \\ \hline
RIDE~\cite{ref:ride_iclr2021}        & 48.6 & 51.4 & 59.8 \\
RIDE + Remix~\cite{ref:remix_eccv2020}               & 44.0 & 47.9 & 59.5 \\
\rowcolor{lightcolor}
RIDE + Ours               & \textbf{50.0} & \textbf{53.0} & 60.2 \\ \bottomrule
\end{tabular}
}
\end{table}


==> tables/old-res-imagenet.tex <==
\begin{table}[]
\caption{
Classification accuracy (\%) of ResNet-50 on ImageNet-LT.
Baseline results are copied from their original paper, and ``$\dagger$" means that the results are from~\cite{ref:causalnorm_neurips2020} and
``$\ast$" indicates that the results are copied from the original paper, 
% and ``$\ddagger$" means that the results are from~\cite{ref:causalnorm_neurips2020} .
The best results are marked in bold.
}
\vspace{0cm}
\label{table:imagenet-lt}
\centering
\small
{
\begin{tabular}{lcccc}
\toprule
                   & All  & Many & Med  & Few  \\ \midrule
Focal Loss~\cite{ref:lin_focal_loss_iccv17}$\dagger$         & 43.7 & 51.0 & 40.8 & 20.8 \\
Decouple-$\pi-$norm~\cite{ref:kang_decoupling_iclr2020}$\dagger$             & 46.7 & 56.6 & 45.2 & 29.3 \\
Decouple-cRT~\cite{ref:kang_decoupling_iclr2020}$\dagger$                & 47.3 & 58.8 & 44.0 & 26.1 \\
Decouple-LWS~\cite{ref:kang_decoupling_iclr2020}$\dagger$                 & 47.7 & 57.1 & 45.2 & 29.3 \\
LDAM-DRW~\cite{ref:cao_ldam_neurips2019} & 49.8 & 60.4 & 46.9 & 30.7 \\
Causal Norm~\cite{ref:causalnorm_neurips2020}$\dagger$         & 51.8 & 62.7 & 48.8 & 31.6 \\
LADE~\cite{ref:lade_cvpr2021}$^\ast$            & 51.9 & 62.3 & \textbf{49.3} & 31.2 \\ \hline
Cross Entropy (CE) & 41.6 & 64.0 & 33.8 & 5.8  \\
CE + Remix~\cite{ref:remix_eccv2020}    & 41.7 & 66.0  & 33.0  &  5.7  \\
\rowcolor{lightcolor}
CE + Ours          & 49.1 & \textbf{67.0} & 42.3 & 20.5 \\
CE-DRW & 50.1 & 61.7 & 47.3 & 28.8 \\
CE-DRW + Remix~\cite{ref:remix_eccv2020} & 48.6 & 60.4 & 46.9 & 30.7 \\
\rowcolor{lightcolor}
CE-DRW + Ours      & 51.4 & 60.8 & 48.6 & 35.5 \\ 
Balanced Softmax (BS)~\cite{ref:ren_bms_neurips2020} & 51.0 & 60.9 & 48.8 & 32.1  \\
BS + Remix~\cite{ref:remix_eccv2020}          & 49.2 & 61.6 & 47.5  & 22.2  \\
\rowcolor{lightcolor}
BS + Ours          & \textbf{52.3} & 62.0 & 49.1 & \textbf{36.7} \\ \bottomrule
\end{tabular}
}
\end{table}

% MiSLAS: 52.7
